SN2019yvq Does Not Conform to SN Ia Explosion Models

We present new photometric and spectroscopic observations of SN 2019yvq, a Type Ia supernova (SN Ia) exhibiting several peculiar properties including an excess of UV/optical flux within days of explosion, a high SiII velocity, and a low peak luminosity. Photometry near the time of first light places new constraints on the rapid rise of the UV/optical flux excess. A near-infrared spectrum at $+173$ days after maximum light places strict limits on the presence of H or He emission, effectively excluding the presence of a nearby non-degenerate star at the time of explosion. New optical spectra, acquired at +128 and +150 days after maximum light, confirm the presence of CaII$\lambda 7300~$\r{A} and persistent CaII NIR triplet emission as SN 2019yvq transitions into the nebular phase. The lack of [OI]$\lambda 6300~$\r{A} emission disfavors the violent merger of two C/O white dwarfs (WDs) but the merger of a C/O WD with a He WD cannot be excluded. We compare our findings with several models in the literature postulated to explain the early flux excess including double-detonation explosions, $^{56}$Ni mixing into the outer ejecta during ignition, and interaction with H- and He-deficient circumstellar material. Each model may be able to explain both the early flux excess and the nebular [CaII] emission, but none of the models can reconcile the high photospheric velocities with the low peak luminosity without introducing new discrepancies.

==> line_params.tex <==

\begin{table}
    \centering
    %\vspace{0.5cm}
    \caption{Non-detections for \Ha and [\ion{O}{1}]$\lambda6300\rm\AA$. }

    \begin{tabular}{lcccc}
    \hline
        Line & Phase & $W_{3\sigma}$ & $F_{5\sigma}$ & $L_{5\sigma}$  \\
         & [days] & [$\rm\AA$] & [$10^{-17}$ erg/s/cm$^2$/$\rm\AA$] & [$10^{37}$ erg/s] \\\hline
        \Ha &  128 & 0.52 & 6.9 & 2.3 \\
         & 150 & 0.55 & 3.3 & 1.1 \\\relax
        [\ion{O}{1}] & 128 & 0.52 & 5.8 & 2.0 \\
         & 150 & 0.94 & 5.1 & 1.7 \\\hline
    \end{tabular}
    \label{tab:line_params}
\end{table}

==> phot.tex <==
\begin{table}
    \centering
    \caption{$r$-band photometry and $V$/$R$/$i$-band spectrophotometry of \name and the computed decay rates per 100 days.}
    \begin{tabular}{cccc}
         Filter &  +128 & +150 & $\gamma$\\
         & [mag] & [mag] & [mag/ 100d] \\\hline
        $V$ & $18.74\pm0.06$ & $19.37\pm0.08$ & $2.8\pm0.3$ \\
        $r$ & $19.03\pm0.04$ & $19.79\pm0.06$ & $3.5\pm0.2$\\
        $R$ & $18.97\pm 0.06$ & $19.56\pm0.07$ & $2.7\pm 0.3$ \\
        $i$ & $18.92\pm0.11$ & $19.42\pm0.13$ & $2.3\pm0.6$ \\\hline
    \end{tabular}
    \label{tab:phot}
\end{table}
